On definite lattices bounded by integer surgeries along knots with slice genus at most 2

We classify the positive definite intersection forms that arise from smooth 4-manifolds with torsion-free homology bounded by positive integer surgeries on the right-handed trefoil. A similar, slightly less complete classification is given for the (2,5)-torus knot, and analogous results are obtained for integer surgeries on knots of slice genus at most two. The proofs use input from Yang--Mills instanton gauge theory and Heegaard Floer correction terms.

==> sections/table-old.tex <==
% !TEX root = ../main.tex

\begin{sidewaysfigure}\small
\centering
\begin{tabular}{*{12}{p{15mm}}}
 $\text{rank}\backslash \text{det}$  & 1 & 2 & 3 & 4 & 5  & 6 & 7 & 8 & 9 & 10 & 11\\
\hline\\
1 &  \textbf{--} \newline ${}$ \newline  & $A_1$  & $O_1$ & $O_1$ & $O_1$ & $O_1$ & $O_1$ & $O_1$ & $O_1$ & $O_1$ & $O_1$\\
2 &  \textbf{--} \newline ${}$ \newline  & \textbf{--}  &  $A_2$ & \textbf{--} & $A_1O_1$  &   \textbf{--}  & $A_1O_1$\hspace{-.75cm}\boxit{.6cm} & $O_2$ & $A_1O_1$ & \textbf{--} & $O_2$\hspace{-.58cm}\boxits{.6cm}\vspace{.08cm} \newline $A_1O_1$ \\
3 &  \textbf{--} \newline ${}$ \newline  & \textbf{--}  & \textbf{--}  & $A_3$ & \textbf{--}  & \textbf{--} & $A_2O_1$ & $A_1^2O_1$ &   \textbf{--} & $A_2O_1$ & \\
4 &   \textbf{--} \newline ${}$ \newline & \textbf{--}  & \textbf{--} & $D_4$ &  $A_4$\hspace{-.55cm}\boxit{.6cm} & \textbf{--} & \textbf{--} & $A_3O_1$ & $A_3O_1$\hspace{-.88cm}\boxits{.6cm} & &  \\
5 &  \textbf{--} \newline ${}$ \newline  & \textbf{--}  & \textbf{--}  &  $D_5$\hspace{-.55cm}\boxit{.6cm} & \textbf{--}  & $A_5$ & \textbf{--} & $D_4O_1$\hspace{-.88cm}\boxits{.6cm} & & & \\
6 &  \textbf{--} \newline ${}$ \newline  & \textbf{--}  & $E_6$\hspace{-.55cm}\boxit{.6cm} & $D_6$ & \textbf{--}  & \textbf{--} &  $D_5O_1$\hspace{-.88cm}\boxits{.6cm}\vspace{0.08cm}\newline $A_6$  &&  &  & \\
7 &  \textbf{--} \newline ${}$ \newline  & $E_7$\hspace{-.55cm}\boxit{.6cm}  & \textbf{--} & $D_7$ & $E_6O_1$  & $D_6O_1$\hspace{-.88cm}\boxits{.6cm}   &&& &  & \\
8 &  $E_8$\hspace{-.55cm}\boxit{.6cm}  \newline ${}$\newline  & \textbf{--}  & $E_7O_1$ & $D_8$ &    $D_7O_1$\hspace{-.88cm}\boxits{.6cm}\vspace{.08cm} \newline $E_7O_1$ & & &&& & \\
9 & \textbf{--}\newline ${}$ \newline  & \textbf{--}  & \textbf{--} &  $D_8O_1$\hspace{-.88cm}\boxits{.6cm} \vspace{.08cm} \newline $E_7A_1O_1$ \newline $D_9$  \vspace{-.4cm}&  & &&& & & \\
10 &  \textbf{--}\newline ${}$ \newline & \textbf{--}  &  $D_9O_1$\hspace{-.88cm}\boxits{.6cm} &  & &  &   &&&  & \\
11 & \textbf{--}\newline ${}$ \newline   &  $D_{10}A_1$\hspace{-.95cm}\boxits{.6cm} &  &  &   &  &&& &  & \\
12 & $D_{12}$\hspace{-.75cm}\boxits{.6cm}  \newline ${}$ \newline &   &   &  &  &  &  &&& & \\
\end{tabular}
\captionof{table}[]{Reduced indecomposable positive definite integral lattices of low rank and determinant taken from \cite{cs-low}. A dash ``\textbf{--}'' indicates that there are no lattices of the associated rank and determinant. The indecomposable distinguished lattices $\mathscr{T}_n$ and $\mathscr{C}_n$ have been boxed.}\label{fig:tableroots}
\end{sidewaysfigure}
